TeaMPI -- Replication-based Resilience without the (Performance) Pain

In an era where we can not afford to checkpoint frequently, replication is a generic way forward to construct numerical simulations that can continue to run even if hardware parts fail. Yet, replication often is not employed on larger scales, as na\"ively mirroring a computation once effectively halves the machine size, and as keeping replicated simulations consistent with each other is not trivial. We demonstrate for the ExaHyPE engine -- a task-based solver for hyperbolic equation systems -- that it is possible to realise resiliency without major code changes on the user side, while we introduce a novel algorithmic idea where replication reduces the time-to-solution. The redundant CPU cycles are not burned "for nothing". Our work employs a weakly consistent data model where replicas run independently yet inform each other through heartbeat messages whether they are still up and running. Our key performance idea is to let the tasks of the replicated simulations share some of their outcomes, while we shuffle the actual task execution order per replica. This way, replicated ranks can skip some local computations and automatically start to synchronise with each other. Our experiments with a production-level seismic wave-equation solver provide evidence that this novel concept has the potential to make replication affordable for large-scale simulations in high-performance computing.

==> 10_notation.tex <==
\section{Notation}

We quickly lay out the notation used. The upper part of the table enlists
constants, the lower part all other variables.


\begin{center}
 \begin{tabular}{l|p{8cm}}
   Symbol & Description \\
   \hline
   $K$  & Replication factor, i.e.~number of teams. \\
   $R$  & Number of ranks. \\
   \hline
   $A,B,C$ & Team identifier \\
   $i,j,k,l$ & Task identifiers, always used as $i^{(A)}$, $l^{(B)}$, \ldots
   depending on the team they belong to. \\
   $r$  & Rank identifier, always used as $r^{(A)}$, $r^{(A)}$, \ldots or
   $r_{1}^{(A)}$,$r_{2}^{(B)}, \ldots$ \\
   $t$, $\Delta t$ & Timestamps and time intervals.
 \end{tabular}
\end{center}

==> tdlb.tex <==
% !TEX root = thesis.tex

\chapter{Conclusion and Synthesis of Contributions}\label{chapter:conclusions}
In this thesis I have presented two novel contributions based upon asynchronous algorithms in high performance computing. The first, enclave tasking, uses a producer-consumer idiom and task fusion to ensure high concurrency on dynamically adaptive meshes. As the approach is naturally suited to an overlapping communication approach, it efficiently scales using a hybrid combination of MPI and TBB\@. It is now used in the {\exahype} project to use the powerful refinement features of the codebase without suffering the severe overheads of the previous parallel-for based implementation.

The second contribution is the {\tmpi} library, which creates asynchronous teams from an applications MPI ranks. After a thorough review of existing approaches, I identified a common weakness in that the strong consistency models used induce extremely fine-grained synchronisation among replicas. Therefore by allowing the \emph{application} to decide when to ensure consistency, the overhead is drastically reduced to practically zero. The exchange of both performance and consistency information is implemented in a fully non-blocking fashion and allows the {\tmpi} library to detect slow or failing ranks and memory corruption errors without the runtime overhead.

One of the key challenges of the approach outlined in Chapter~\ref{chapter:tasks} is ensuring that each rank has an equal amount of tasks to execute. If one has a larger portion of the computational domain then other ranks with less work will have to wait and their computational resources wasted. Optimal domain decompositions with dynamically adaptive grids is a complex topic, as the work per rank may frequently change. This means any decomposition is unlikely to remain valid for long. 

I now provide an outlook into a future area of research that combines the two contributions of this thesis into an idea called team-based diffusive load balancing. 

The {\tmpi} library assumes that if replicas are consistent at every heartbeat then they must have executed roughly similar instructions. The final state of all replicas is identical. With TDLB, the consistency model is weakened further such that the replicas no longer operate identically. However, the heartbeat's still mark points where the replicas can compare state.

I outline a use case for this with respect to {\exahype}. Even if we assume that each cell requires the same amount of time to process, which in the case of non-linear problems is not true, the distribution of work is still non-trivial. If cells are refined or coarsened throughout the simulation then the amount of work on that process will change. This leads to the two challenges to tackle: firstly how to detect the load imbalance detected and secondly how to resolve the imbalance. Existing approaches to the first usually involve abstracting the work into a cost model, which in this case could be the number of cells per rank~\cite{schaller2016swift}. In {\tmpi} we can do better and use the real measurements provided by the heartbeat performance consistency features.
 

The more challenging, and still an active research area, is how to then rectify the load imbalance? Two main approaches exist. The first requires the application to send and receive cells between ranks as and when required by the load balancer~\cite{peano15}. This approach requires the application to stop and redistribute the work which invokes considerable overhead through synchronisation and data transfer costs. The second approach allows ranks to steal ``tasks'' from each other and then send the result back~\cite{CharmPDAABook09,samfass17towards,samfass18parallel,samfass18stealing}. If this happens too often they then do an actual redistribution. However, the issue with both approaches is that data transfer is often considered to be the bottleneck of exascale applications. TDLB is designed to be a data-conservative load balancing scheme.


The core idea of TDLB is for replicas to host \emph{some} cells redundantly, modelling classical overlapping domain-decomposition. However, only a subset replicas will maintain a valid state for a cell. If replicas host the same cells then in {\exahype} with the contributions from Chapter~\ref{chapter:tasks} they will spawn the same tasks into their queues. In the experiments in Section~\ref{section:teams:exahype} this means that each replica executes the same STP tasks, an equal amount of work.


However, if the replicas grids do not completely overlap then only some of the STP's are spawned redundantly. With TDLB a heatmap could be embedded into the computational grid. The value in the heatmap would dictate how likely a rank is to provide the result for that cell. Some cells the replica will completely own, and it can process the tasks as normal. Other cells will be owned by multiple replicas, and each send around the result of those cells between each other. On receiving the result of a STP, it can be compared using {\tmpi}'s data consistency features. Throughout the simulation, the overlap will be reduced such that the redundancy in the computation is eliminated.

To summarise, I have presented two novel contributions. In Chapter~\ref{chapter:tasks} I investigate a lightweight, asynchronous distributed task system for Discontinuous Galerkin applications. By prioritising critical tasks and efficiently balancing resource usage it promises good scaling even for heavily dynamic adaptive grids up to hundreds of cores. In Chapter~\ref{chapter:teams} I introduce the {\tmpi} library that replicates MPI ranks to form teams. These teams are able to operate with minimal communication overhead using a novel heartbeat-based consistency scheme. Additional features include the option to efficiently detect data or performance issues for individual ranks. Finally I show that these two contributions can be brought together with future research surrounding a team based diffusive load balancing scheme. With teams able to share tasks, load can be balanced dynamically at runtime allowing for increasingly complex applications to scale on the worlds largest machines.  

==> teampi.tex <==
% !TEX root = thesis.tex

\chapter{Asynchronous Teams}\label{chapter:teams}
In many areas of large-scale computing, the success of a given approach is preliminarily dictated by the performance. At exascale, a second success factor enters the game: fault tolerance. Although quantifying the performance of a given solution is usually trivial, proving a tolerance to ``faults'' is challenging. Faults in this thesis refer to errors in hardware, such as outright failures or ``silent'' memory faults that produce erroneous results. Barring HPC, almost every other field uses the idea of replicated resources to ensure that maximum performance is achieved even when faults occur~\cite{Cappello2009}. For example, cloud computing, sensor networks, desktop grids and peer-to-peer networks all base their fundamental fault tolerance capabilities upon the idea of replicating resources. Traditionally HPC has relied on a technique called \emph{checkpoint-restart}. It requires applications to periodically save their state to an external storage medium that can be loaded in the case of a failure. Faults then reduce the efficiency of an application, forcing rollbacks previously saved states. The success of this approach is owing to three assumptions that have remained valid over the past 40 years~\cite{Ferreira2011a}.
\begin{enumerate}
	\item Application state can be saved and restored much quicker than a system’s mean time to interrupt (MTTI);

	\item the hardware and upkeep (e.g.\ power) costs of supporting frequent check-pointing are a modest  (perhaps 10--20\%) compared to the system’s overall cost; and
	\item system faults that crash (fail-stop) the system are rare.
\end{enumerate}

Work over the past decades in checkpoint recovery has largely focused on keeping these statements valid. However, each one is challenged by exascale. Although the mean time before failure of a single node is measured in years, combining the large amount of nodes required to form an exascale machine reduces this value dramatically. This is a troubling issue when the purpose of such machines is to allow for much larger experiments to be carried out, which naturally increases the time required to write a checkpoint. Several theoretical studies have been carried out in the past decade that validate with current failure rates, replication will be mandatory for an exascale application~\cite{Riesen2010,Ferreira2011a,Engelmann2009,Bougeret2013,engelmann2014scaling}. Without it, exascale machines will spend most of the time writing and recovering from checkpoints rather than computing ``useful'' results. This is achieved by modifying existing scaling models such as Amdahl's~\cite{amdahl1967validity} and Gustafason's~\cite{gustafson1988reevaluating} Laws to include reliability as outlined by Zheng and Zhiling~\cite{Zheng2009}.


 

In the exascale software roadmap by Dongarra et al~\cite{dongarra2011international}, replication is again raised as a potential solution to the fault-tolerance challenges at exascale. Following up on these ideas, several empirical studies presented implementations of process replication and a thorough review is undertaken in Section~\ref{section:lit-review}.




In addition to (unpredicted) increasing hardware reliability, the issue process replication faces to this day is that multi-million Dollar investments into exascale computing is a difficult sell for vendors when requiring 2--3x redundant computation. Replication based fault tolerance has since fallen out of fashion, replaced instead by approaches that catch or mitigate faults. Run-through-stabilisation techniques pioneered by the ULFM-MPI project~\cite{bland2013ulfm,fagg2005process,chen2005fault} allow applications to use new MPI features to continue running even when a process fails. Another alternate ideas include process migration teamed with failure prediction. Faults are predicted using advanced detection techniques and processes are migrated before it occurs. Although a large and promising research field, it is still not capable of handling all errors and therefore still relies upon traditional methods~\cite{Chakravorty2006,wang2008proactive,Schroeder2010,Schroeder2007,gainaru2013failure,zheng2010practical,gainaru2012fault,gainaru2012taming}.




The replication research proposed here will tackle, in parallel, another major show-stopper raised in the exascale roadmap: heterogeneous system performance. Even individual nodes may differ by up to 10\% through effects such as component binning and heat. Therefore, one of the main contributions of this project will be how this imbalance can be reduced with replication. Clearly,for process replication to be adopted it must also provide resilience without performance deficits.
 
\begin{figure}%
	\centering
	\includegraphics[width=0.75\linewidth]{figures/tmpi-stack.eps}
	\caption[{\tmpi} software stack.]{The layers of a proposed software stack involving the {\tmpi} library. Both ExaHyPE and Peano are optional. If the {\tmpi} layer is removed the application will function identically to when replicated.}
	\label{fig:stack}
\end{figure}%
In this chapter I present a new library, {\tmpi}, in which \textbf{tea}ms of \textbf{MPI} processes are created transparently from the application to provide fault tolerance and detect performance issues of team members. I first define some of the key terms that will be used throughout the chapter. Since the original idea of replicating MPI processes is not new I carry out a literature review of the existing implementations in Section~\ref{section:lit-review}. After a critical analysis of these approaches, I introduce my library and its novel approach surrounding teams \emph{without synchronisation} in Section~\ref{sec:progress}. This has several advantages over existing approaches such as the ability to detect faults and performance issues of individual ranks with minimal overhead, as discussed in Section~\ref{sec:tmpi:results}. The chapter ends with some concluding remarks. 

\begin{tcolorbox}[colback=white,colframe=blue!75!black,title={\tmpi} overview]
	Rank replication is enabled by splitting a global pool of ranks into distinct sub-pools called teams. Each team operates as a separate instance of the application by exchanging messages through a new communicator. At application-defined points, named heartbeats, the teams asynchronously exchange information to compare the states of data and performance. 
  \end{tcolorbox}


\section{Review Of Existing Approaches}\label{section:lit-review}
A review in the area of existing replication work investigates the challenges faced by previous implementations and the solutions each one presents. As the number of such projects is large and vary with intended use, the focus is on supporting process replication in an MPI environment used by most scientific computing codes. First, I explain the core features common to all approaches. As each share a common goal each naturally share features. However, the approaches differ in each project with varying degrees of success. In Section~\ref{section:lit-review:existing}, I next introduce the projects and which features they pioneered or innovated. Finally, the strengths and weaknesses are critically evaluated to direct the contributions of this project. 

\subsection{Integration Of Replication}\label{sec:lit-review:integration}
In all the existing work I found, the underlying replication is transparent to the user's application. This is common to many other areas of replication, such as the RAID data storage virtualization technology. When saving files redundantly it is not necessary for the user to know that these multiple copies exist. 

To realise this, MPI replication is implemented as a library that intercepts MPI calls to handle the replication internally. The requirement to intercept MPI calls is not unique to this area, therefore MPI libraries provide a dedicated ``profiling'' interface: PMPI\@. The profiling layer of MPI is designed such that libraries can intercept the calls to the MPI library and execute arbitrary code instead. Usually the interceptor forwards the MPI invocation to preserve the function's semantics. The MPI standard requires that the core functionality be provided by ``name shift'' functions prefixed by an upper-case P\@. Each function is declared twice. For example, \texttt{MPI\_Send} is also declared as \texttt{PMPI\_Send}. 

MPI library implementers have two approaches given by the standard to provide this interface. If the compiler and linker support weak symbols (as most modern systems do), then the original MPI functions can be weakly defined. At link time the symbols are overridden if another library provides a ``strong'' definition for them.  When an application calls \texttt{MPI\_Send} (or any other function declared in the libraries' header) the definition is provided by the library. The original functionality of \texttt{MPI\_Send} is then available via the \texttt{PMPI\_Send} interface.  

The other solution relies on the C macro preprocessor, and therefore the library cannot be added at link time. I do not outline this usage here as it is not required for modern systems. Interested readers are directed towards Section 14.2 (Profiling Interface) in the MPI Standard~\cite{MPI:15}.

For replication, this allows libraries to operate completely transparently. If an application requests the number of ranks available to it through \texttt{MPI\_Comm\_size}, the library can simply return the value given by \texttt{PMPI\_Comm\_size} and divide by the level of replication. 

One of the main disadvantages of the profiling layer is that it can only be used by a single library at a time. Only one may intercept the MPI calls. A workaround is provided by the P\textsuperscript{N}MPI project~\cite{schulz2006flexible,schulz2007pn}, which allows multiple applications to use the profiling layer concurrently. Another potential downfall for library developers is that with hundreds of MPI functions, missing out any will result in application bugs. Thankfully, it is possible to generate the interface for a library automatically using the wrap script developed by Gamblin~\cite{wrap}. 

\subsection{MPI Consistency}
For any area of replication, keeping the state of replicas \textit{consistent} is an important topic. Specifically for MPI, the state refers to the result of calculations and the data sent between ranks. It must be identical among replicas. Existing approaches adopt ideas from the wider field of fault tolerance, using active or passive replication. Active replication is the scheme used by most, where messages are sent to all replicas. This is in contrast to passive replication where a master replica is chosen that then broadcasts results to slave replicas. 

Two main protocols exist to ensure replicas remain consistent: mirror and parallel (Figure~\ref{fig:consistency}). 


\begin{figure}%
	\centering
	\captionsetup[subfigure]{justification=centering}
	\subfloat[][Parallel\label{fig:consistency:parallel}]{{\includegraphics[width=.45\linewidth]{figures/parallel-consistency.eps} }}%
	\hfill
	\subfloat[][Mirror\label{fig:consistency:mirror}]{{\includegraphics[width=.45\linewidth]{figures/mirror-consistency.eps} }}%
	\caption[Parallel and mirror message consistency protocols.]{A comparison of the parallel and mirror consistency schemes. There a two ranks, A and B, with a replication factor of two. Rank A sends a message to rank B. The mirror mode must ensure that the ordering of messages is identical for wildcard receives. Parallel mode must additionally acknowledge that the messages were received.\label{fig:consistency}}
\end{figure}%

\begin{definition}{Mirror Consistency Protocol}{mirror}
	Each message is duplicated to all replicas redundantly. For each message $r^2$ are sent in total, where $r$ is replication factor.  
\end{definition}

\begin{definition}{Parallel Consistency Protocol}{parallel}
	Each message is only sent to the corresponding replica. For each message $r$ are sent in total, where $r$ is replication factor. 
\end{definition}

The mirror protocol requires ranks to send/receive from all of its replicas, whereas in the parallel mode ranks only send/receive with their respective replica pair. Mirror sends \( m \cdot r^2 + c \) messages, where $m$ is the number of original messages, $r$ is the replication factor and $c$ is the small messages sent to ensure consistency among replicas. The parallel protocol is more bandwidth efficient, sending only $m\cdot r + c$  messages. However, the parallel protocol has to send many more messages than the mirror protocol to ensure consistency. This leads to a much larger value of $c$.

The mirror protocol only has to send extra small messages to ensure that MPI behaves identically across replicas. Certain features of the MPI standard are allowed to behave non-deterministically. Non-deterministic message passing means that a message may not be sent the same way in two different runs of the application. This subset of MPI functions raise issues with ensuring consistency among replicas, as executing the same code on each replica may return different results. The first example of this is the \texttt{MPI\_ANY\_SOURCE} parameter in receive operations, that could allow replicas to receive messages in differing orders. Other features which exhibit similar properties include: \texttt{MPI\_Wtime}, \texttt{MPI\_Probe}, and \texttt{MPI\_Test}. The replicas communicate to ensure that the operation occurs identically. 

The parallel consistency mode must also ensure that messages are sent. This requires introducing many small messages into the system testing for completed operations, but reduces the strain on the network bandwidth.

Micro-benchmarks that are either bandwidth sensitive or message rate sensitive stress both the mirror and parallel consistency schemes respectively. The mirror protocol suffers from large message sizes due to bandwidth constraints whereas the parallel protocol suffers from small message sizes sent at high rates where latency becomes a bottleneck~\cite{Ferreira2011rmpi}. When tested with multiple real world applications, it was clear that most exhibit properties of the former, with larger messages sent less often. Therefore the overhead of the mirror protocol is much larger than the parallel protocol for many real world applications. 

Passive replication is less popular for MPI, used by only a single previous implementation. This is because the result of operations must be broadcast to the cloned slaves. Although it allows a library to easily vary the number of replicas per rank, the increased latency is too greater price to pay. 

\subsection{Previous implementations}\label{section:lit-review:existing}
In total I found five existing implementations matching my criteria, each taking a different approach to provide replication. Two projects, rMPI and MR-MPI, merged to form redMPI\@. None of the existing approaches are under active development, or to the best of my knowledge, supported still.
\subsubsection{rMPI}\label{sec:rmpi}
The rMPI project was the first empirical study on replicated MPI processes and operates using the PMPI~\cite{Ferreira2011rmpi}. In theory this should allow rMPI to work regardless of MPI version. However, the prototype includes a number of MPICH specific function calls to implement collective operations in a point to point manner and as a result is tied to a fixed version of MPICH\@. This is likely a result of being first out of the gate, as a number of competing implementations were also released following rMPI in 2011. After reiterating the need for examining replication as a solution for resilience, the authors dive into the practical details of replicating MPI process by introducing the two supported active consistency modes: mirror and parallel.

The library differentiates between master and replica messages by flipping the higher order bit of the message tag. The implementation is therefore limited to only duplex replication. It is also unable to support the simultaneous use of the \texttt{MPI\_ANY\_TAG} and \texttt{MPI\_ANY\_SOURCE} parameters. Finally, it relies on the commonly valid assumption that the underlying MPI implementation supports tags larger than the $2^{15}$ required by the standard.


\subsubsection{MR-MPI}\label{sec:mrmpi}
The modular redundancy MPI project (MR-MPI) from Oak Ridge National Laboratory~\cite{engelmann2011redundant} can be seen as a polish of the rMPI prototype, freeing itself from a number of its predecessors limitations. Although MR-MPI only supports the mirror protocol, it is MPI implementation independent and supports arbitrary replication, both fixed and partial. With partial redundancy, some ranks may have more replicas than others. MR-MPI also natively supports collective operations by using the \texttt{MPI\_Reduce\_local} function. Ultimately, performance results from their work largely mirror the findings from the rMPI project. 

\subsubsection{redMPI}\label{sec:redMPI}
The redundant MPI (redMPI) project is a collaboration merging the two previous libraries: rMPI and MR-MPI~\cite{elliott2012combining,boehm12file}.

Although work on rMPI and MR-MPI carried out performance testing and provided some initial results, there were many unanswered questions from the theoretical studies to tackle. First, the authors define a mathematical model to demonstrate the effectiveness of replication combined with checkpoint-restart over the pure check-pointing solution~\cite{elliott2012combining}. MR-MPI did include partial redundancy, so redMPI did too. However, after an investigation it was found to not be an effective solution for fault tolerance. The second focussed on error detection and correction~\cite{fiala12detection2}. In this paper the authors define a new approach where replicas only send an envelope containing a hash of the message content rather than the actual message. If a replication factor of two is used, the error can be detected if the two hashes are different. A replication factor of three allows for error correction as the correct result can be decided by a simple voting mechanism. This assumes errors are rare and therefore only one replica will be at fault.  

\subsubsection{EchoMPI}
The EchoMPI project~\cite{cobb2011mpiecho} was also released in 2011, but adopted a consistency scheme from fault tolerance traditionally known as passive replication in other fields. It is another library that proves the versatility of the PMPI, providing a library that is independent of the MPI implementation used. Passive replication implies that the state from one replica is transferred to all others. The library introduces the concept of ``master ranks'', which broadcast the result of MPI operations to ``clone ranks''. This allows for arbitrary yet simple replication of individual ranks, but introduces much larger latency overheads. Although a message only has to be sent once among master ranks, it must then be broadcast to the clones. Therefore limited bandwidth is save at the expense of much high latency. The clones still do all computation, as the necessary data is received from the respective masters. To ensure complete coverage of the MPI library, the EchoMPI interface is generated using wrap~\cite{wrap}. The authors present future use cases for this style of replication such as parallelising heavyweight profiling tools, investigated in a follow-up paper~\cite{rountree2013parallelizing}.

\subsubsection{Send Determinism Replication (SDR-MPI)}
The SDR-MPI project developed at INRIA differs to those discussed previously in that it trades transparency and portability for simplicity and performance~\cite{lefray2013replication}. SDR-MPI modifies the MPI implementation, OpenMPI, to provide the consistency among replicas. It then enforces an ordering of messages at a lower level which requires marking the start and end of each communication between ranks. Although it increases the efficiency of the mirror protocol, the requirement of a patched MPI library is not worth the marginal gains. 

The authors then later extend this implementation to allow replicas to share tasks among themselves with custom constructs~\cite{ropars2015efficient}. Applications create tasks through an API and define sections in which they are executed. Within the section, tasks are shared among replicas such that computation is not performed redundantly. At the end of each section the replicas coordinate their results. 

Three issues exist with the SDR-MPI approach. First, as soon as the replicas no longer carry out computation redundancy then all benefits of replication-based fault tolerance are eliminated. Second, the work is split statically and does not take into account heterogeneity among tasks. Finally, it requires applications to be rewritten in a task language using their API and a custom MPI library. This imposes a lot on the applications developers. 

\subsection{The takeaways from existing approaches}
\begin{table}
	\centering
	\caption{Feature comparison of existing rank replication approaches.\label{table:comparison}}
	\begin{tabular}{l*5c}
		\toprule
		                    & rMPI   & MR-MPI & RedMPI & echoMPI & SDR-MPI    \\
		\cmidrule(lr){1-6}
		Fixed replication   & \cmark & \cmark & \cmark & \cmark  & \cmark     \\
		Partial replication &        & \cmark & \cmark & \cmark  &  \\
		PMPI & \cmark & \cmark & \cmark & \cmark \\
		Error correction    &        &        & \cmark & \cmark  &            \\
		Work-sharing         &        &        &        &         & \cmark     \\
		Overhead (1--5)      & 3/4    & 3/4     & 3/4     & 5       & 2          \\
		\bottomrule 
	\end{tabular}
\end{table}
A summary of the comparisons is presented in Table~\ref{table:comparison}. The first project to benefit from existing work was the redMPI project, which analysed the strengths and weaknesses of its predecessors (rMPI and MR-MPI), forming a much improved library with a superset of useful features. 

The first major learning point from the literature is that a ``mirror mode'' approach is problematic in a high performance environment because of the extra bandwidth overhead it incurs. Even though the ``parallel mode'' is a much smarter approach, the existing implementations add too much latency overhead by excessively communicating among replicas. In Section~\ref{sec:progress} I introduce a novel idea to drastically reduce the impact of this.

The second takeaway, specifically from the redMPI project, is that partial replication is not likely to be a useful feature as the authors discuss in~\cite{elliott2012combining}. As the location of errors is usually unpredictable, it neither helps with resilience nor performance and only adds complexity. Therefore we do not build this feature into the library.

From the echoMPI library it is clear to see that an enforced master-clone topology with traditional passive replication is also not a suitable candidate in a high performance environment. The requirement to broadcast every result to clones and have an MPI communicator per rank is much too heavyweight. It is conservative in bandwidth overhead but adds large latencies per message. Although the benefits of this approach is that fine-grained replication can be achieved, as previously noted this is unlikely to be required. Clearly, the passive replication approach from classical fault tolerance is not a good fit for high performance applications. Instead an active scheme should be adopted where the replicas are responsible for their consistency, effectively resembling the parallel replication protocol.

The SDR-MPI project shows the potential of work-sharing among replicas, but the extensive changes to user code and the underlying MPI library nullify any potential use cases. In this work, I show that it is possible to get the same increase in performance with a PMPI wrapper that requires much less modification of user code. 

\section{The {\tmpi} Library}\label{sec:progress}
In this section I discuss the architecture and some key design decisions surrounding the {\tmpi} library. The implementation builds upon the lessons learned from studying the previous projects in Section~\ref{section:lit-review}: the replication should be as lightweight and transparent as possible. To deliver the replication, a C++ library is implemented in the MPI profiling layer (PMPI) similar to the existing implementations in the literature and is detailed in Section~\ref{sec:lit-review:integration}. In contrast, the SDR-MPI project requires applications to change large amounts of code to enable replication. Using the PMPI layer provides two key advantages: (i) there is no requirement to modify the existing application code and (ii) allows the library to operate independently from the underlying MPI library implementation.

\begin{algorithm}
	\caption{Splitting the {\commworld} communicator into teams.\label{alg:tmpi-split}}
	\begin{minted}{c}
		// Duplicate MPI_COMM_WORLD first following recommended practise
		PMPI_Comm_dup(MPI_COMM_WORLD, &TMPI_COMM_DUP);
		PMPI_Comm_size(TMPI_COMM_DUP, &world_size);
		PMPI_Comm_rank(TMPI_COMM_DUP, &world_rank);
		team_size = world_size / number_of_teams;
		// Calculate which team this rank belongs to
		int team = world_rank / team_size;
		// Split TMPI_COMM_DUP into number_of_teams sub-communicators
		PMPI_Comm_split(TMPI_COMM_DUP, team, world_rank, &TMPI_COMM_TEAM);
		// New rank and size returned to the application when called
		PMPI_Comm_rank(TMPI_COMM_TEAM, &team_rank);
		PMPI_Comm_size(TMPI_COMM_TEAM, &team_size);
	\end{minted}
\end{algorithm}

The main idea of building the teams is to split a pool of ranks into teams of replicated ranks. The application has no knowledge that these replicas exist. The ranks are mapped into $t$ equal sized teams of contiguous processes, lines 7--9 of Algorithm~\ref{alg:tmpi-split}. This default mapping can easily be modified to any one-to-many function. To separate and de-synchronise replicas, the original MPI communicator {\commworld} is first duplicated for preservation, as recommended by the MPI standard for libraries, then split into $t$ sub-communicators. Each team then has access to a separate communicator, {\commteam}, for messages that would usually get sent via {\commworld}. This means that identical messages sent by different teams are not subject to the strict message ordering imposed by MPI, where messages of the same tag and communicator cannot overtake. The code snippet for splitting the communicator into teams is given in Algorithm~\ref{alg:tmpi-split}.
\begin{algorithm}
	\caption{The \texttt{MPI\_Recv} function in the {\tmpi} library.\label{alg:tmpi-recv}}
	\begin{minted}{c}
std::map<MPI_Comm, MPI_Comm> commMap;
int MPI_Recv(void *buf, int count, MPI_Datatype datatype, 
              int source, int tag, MPI_Comm comm, MPI_Status *status)            
{
  // Map communicator, e.g. MPI_COMM_WORLD -> TMPI_COMM_TEAM                 
  comm = commMap[comm]; 
  // Perform receive with correct replica of source rank
  // No synchronising consistency checks here! 
  return PMPI_Recv(buf, count, datatype, source, tag, comm, status);
}
	\end{minted}
\end{algorithm}


An advantage of splitting the original communicator is that the mapping between real and logical rank identifier is handled automatically the MPI library. As a consequence, this greatly reduces code complexity as many of the original MPI functions do not require large modifications. For all communication based functions the only change required is to map the provided \texttt{comm} parameter to one split for use in teams.  If {\commworld} is used, then it is a simple mapping to {\commteam}. However, if the application makes use of other communicators by splitting {\commworld} then {\commteam} must also be split in the same manner. When an application splits the {\commworld} communicator, the library splits the {\commteam} communicator and stores the updated mapping in a \texttt{std::map\textless MPI\_Comm, MPI\_Comm\textgreater}. The \texttt{MPI\_Recv} wrapper function is given in Algorithm~\ref{alg:tmpi-recv}, where the only change is the communicator mapping. This also retains the correct values in the \texttt{MPI\_Status} object. For example, the \texttt{status$\rightarrow$MPI\_SOURCE} field will automatically return the team rank of the source, not the global one.  Other implementations such as rMPI instead are forced to make large changes for many functions. In rMPI each collective operation is replaced with a reduced efficiency point-to-point counterpart. The \texttt{MPI\_SOURCE} field of \texttt{MPI\_Status} objects must also be manually altered. Comparisons to other approaches cannot be made as each one does not publish their lower-level implementation details or make their code open source.

\subsection{The heartbeat consistency model}\label{section:teams:zero-overhead}

One of the key differences with the {\tmpi} library compared to the approaches detailed in Section~\ref{section:lit-review} is in the way it ensures consistency among replicas. In all the existing libraries I investigated, each one enforces a \emph{strong} consistency model (Definition~\ref{definition:strong-consistency}).

\begin{definition}{Strong Consistency}{strong-consistency}
	The state of replicas is identical at every MPI function call.
\end{definition}


This causes multiple issues, such as making sure that replicated non-blocking messages complete identically and that messages are received with the same source/tag where wildcards are used.  The paper introducing rMPI is an excellent collection of the issues faced by this model~\cite{Ferreira2011rmpi}, are also discussed in Section~\ref{sec:redMPI}. Additionally, implement the mirror mode as it more naturally supports fault tolerance (Definition~\ref{definition:mirror}, Figure~\ref{fig:consistency:mirror}). However, the quadratic relationship between the messages and replication factor means that the bandwidth required is too high for the majority of codes. Network bandwidth is often a critical resource for HPC applications. Therefore I implement the parallel scheme, which only increases the bandwidth directly proportional to the number of teams. The rMPI project reported that this introduced many small messages into the MPI subsystem to ensure the other replica had sent its message. For \texttt{MPI\_ANY\_*} wildcards it also induces excessive synchronisation as the replicas must ensure each receive from the same source/tag. 

\subsubsection{Weakening the consistency model}
\begin{definition}{Weak Consistency}{weak-consistency}
	The state of replicas is identical only at application defined points (heartbeats).
\end{definition}

One of the core contributions of this work is that I weaken the consistency model (Definition~\ref{definition:weak-consistency}). Most applications do not need to ensure a consistent state among replicas on every MPI function call. Provided that the code uses MPI in a deterministic way, then linking against the {\tmpi} library will not lead to a change in the runtime behaviour. If the code uses non deterministic features such as \texttt{MPI\_ANY\_SOURCE}, then this statement may not hold. For example, if a receive is posted with a \texttt{MPI\_ANY\_SOURCE} source parameter the following may happen: one replica receives a message from rank $x$ while another replica receives a message from rank $y$ first. However, I assume that by the end of the iterations this will have no effect on the \emph{overall} application consistency. The outcome is eventually deterministic. 

\begin{definition}{Heartbeat}{heartbeat}
	An asynchronous operation carrying data to compare the states of replicas. 
\end{definition}

Teams operate fully asynchronously, such that one may advance much further through the execution than others. Applications are only required to check-in via a ``heartbeat'' every so often, usually per iteration (Definition~\ref{definition:heartbeat}). As a ``heartbeat'' operation is performed fully asynchronously, it does not hold faster teams back. To keep integration cost of the library as minimal as possible for the user, this heartbeat can be inserted with a single line of code and still allows the code to compile and run as normal without linking to the {\tmpi} library. 

\begin{algorithm}
	\caption{The \texttt{MPI\_Sendrecv} function in {\tmpi}.\label{fig:heartbeat-signature}}
	\begin{minted}{c}
int MPI_Sendrecv(const void *sendbuf, int sendcount, 
MPI_Datatype sendtype, int dest, int sendtag,
void *recvbuf, int recvcount, MPI_Datatype recvtype,
int source, int recvtag, MPI_Comm comm, MPI_Status *status) 
{
	int err = 0;
	if (comm == MPI_COMM_SELF) {
		if (sendcount == 0) { // Consistency buffer not provided
			err |= heartbeat(sendtag);
			} else { // Consistency buffer provided
			err |= heartbeat(sendtag, sendbuf, sendcount, sendtype);
		}
		} else {
		// Perform actual SendRecv (unmodified parameters omitted)
		err |= PMPI_Sendrecv(..., mapComm(comm),status);
		mapStatus(status);
	}
	return err;
}
	\end{minted}
\end{algorithm}

\subsubsection{Heartbeat Implementation}
The heartbeat is realised via ``hijacking'' the \texttt{MPI\_Sendrecv} function call such that with when passed \texttt{MPI\_COMM\_SELF} as a communicator parameter it operates as the heartbeat (Figure~\ref{fig:heartbeat-signature}). {\tmpi} can differentiate between heartbeats and calls with the original semantics. Since a \texttt{MPI\_Sendrecv} with the host rank (i.e.\ using \texttt{MPI\_COMM\_SELF}) is nonsensical, this is a safe choice. If for some reason an application does require this functionality, {\commworld} can safely be used. The semantics also imply a local operation. This function accepts many arguments with some perfect to leverage for {\tmpi}\@. The implementation of this heartbeat will be covered in the remainder of this section. However, for now it is enough to know that the heartbeat is fully asynchronous (a regular \texttt{MPI\_Sendrecv} operation is still blocking) and consumes very little bandwidth. First, I outline two initial uses of the heartbeat consistency scheme, the detection of (i) slow or (ii) faulty ranks. Then I show that the overhead of such a consistency scheme is minimal in most cases. 

\subsubsection{Measuring performance homogeneity via heartbeats}\label{sec:compare-progress}
\begin{algorithm}
	\caption{Compare progress of replicas}\label{alg:progress}
	\begin{algorithmic}[1]
		\Procedure{compareProgress}{}
		\For {replica of this rank}
		\State \texttt{Isend} current time to replica
		\State Post \texttt{Irecv} for time from replica
		\EndFor
		\State \texttt{MPI\_Testsome} on pending requests check and progress received times
		\State Process times which have been received
		\EndProcedure
	\end{algorithmic}
\end{algorithm}

The first intended use of the heartbeat consistency scheme is to detect slow ranks within a team. In Section~\ref{sec:tmpi:results}, I show that this can pollute the performance of applications. Such slow ranks can be considered close to broken where a slow-down is a precursor to a failure.  In general this means {\tmpi} must detect the performance variations among replicas. By comparing the heartbeat times among replicas it is then possible to detect if one is falling behind the others. This could be due to any number of factors such as variations in processor binning, heat levels or network traffic. Other replication libraries have no simple way to measure this because of the strict consistency protocols, where the states of replicas are synchronised at each MPI function call. Therefore it would have to be done on a much finer level at each function call which would introduce many small messages into the network sub-system. For example, measure which team reaches an \texttt{MPI\_Wait} call first. This approach however will struggle to detect long running issues in ranks and will be sensitive to small variations in the individual runtime behaviour of ranks such as operating system interference. It also introduces extremely tight coupling between teams.

With {\tmpi}, the heartbeats are piggy-backed to carry timestamps. As mentioned previously, most scientific codes are iteration or loop based and therefore inserting the regular \texttt{MPI\_Sendrecv} commands is just a single line addition in the loop body. Algorithm~\ref{alg:progress} outlines the steps required to compare the progress of replicas asynchronously using MPI non-blocking communication. It is imperative that synchronisation is avoided among ranks, in this case specifically replicas, so the library supports two modes of asynchronous communication. The first is used when the underlying applications supports the eager send protocol. Eager sends are where the data to be sent is transferred to a temporary buffer on the receiver until the matching receive is posted. It is then copied into the supplied buffer. Owing to memory and copy overhead on the receiver side, eager sends are only supported for small messages. The default threshold for the Intel MPI library is 256kB, for which the heartbeat messages easily fall under. If the receive is posted before the send then the \texttt{MPI\_Testsome} operations ensure that the previously posted receives get completed. If eager sends are not supported by the MPI library or disabled by the user for their application, then these \texttt{MPI\_Testsome} operations become important for making sure that heartbeat communication completes. This is known as manual progression of MPI messages~\cite{Hoefler:08:SacrificeThread}, and plays an important role in the contributions outlined in Chapter~\ref{chapter:tasks}.

How to process the received times is flexible. The simplest way is to compare the latest time and if one replica exceeds a set tolerance then it is marked as ``slow''. At this point the faster team could checkpoint it's state at the next heartbeat. Then the single slow rank of team can be swapped out for another. Making a decision based upon a single time interval is likely not a wise idea with the significant overhead of swapping processes. Instead, more advanced statistical techniques may be employed on the entire history of replica timings. For example, exponential smoothing is a commonly used technique used on time series data where older data is considered with less importance. If a process becomes temporarily slow but manages to recover then the old ``slow'' times will be outweighed by the recent improved performance. Another approach could be to detect if a process frequently suffers from small slow-downs but then recovers. Such minor slow-downs will not impact the runtime if taken on their own but added together but overall could drastically reduce progress for a team.  Clearly, a range of models should be investigated and is a future research topic.

When first testing the single heartbeat idea I discovered a large drawback in its ability to detect a slow \emph{rank}. Although many scientific codes are \emph{iteration} based, there is usually some synchronisation per iteration such as a neighbour communication step or a global collective. The frequency of the synchronisation points depend on the parallelisation properties of the algorithm. Coarse-grained algorithms are able to go longer before synchronising ranks. The consequences for the heartbeat approach is that if one rank is slow, it will also hold back the other members of the same team while they wait for that rank to complete the iteration. With a single heartbeat, it is then impossible to know the offending slow rank, as the whole team will report a slow heartbeat. Therefore I propose a more effective technique, inserting \emph{two} heartbeats into the application code. This time, care must be taken to ensure the two heartbeats are in suitable locations. There must be no synchronisation with other ranks between heartbeat pairs. Although this seems like a large constraint at first, most applications aim to be as coarse-grained as possible. In Section~\ref{sec:tmpi:results}, I present a trivial application of this idea and then show how it can also be introduced into a highly complex application such as {\exahype}.

\begin{figure}
	\centering
	\includegraphics[width=\textwidth]{figures/performance-consistency.eps}
	\caption[An illustration of the heartbeat process for performance consistency data.]{An illustration of the heartbeat process with two teams for performance consistency data. The first team is faster than the second. When team 1 triggers the heartbeat for tag 2 of $h_1$, the data is sent back to team 0 which had already posted the receive. Green indicates a completed communication. Red indicates a pending communication.}\label{fig:performance-consistency}
\end{figure}

To switch between the single and dual heartbeat modes I use the \texttt{sendtag} parameter of the \texttt{MPI\_Sendrecv} function. A positive tag value starts a heartbeat and a negative tag value ends it. Multiple heartbeats allow {\tmpi} to measure the times for various sections of code can be introduced with unique tag values. This is therefore a flexible approach. A tag value of zero signals to the library that the single heartbeat algorithm should be used. In the library the data is stored in map data structure. A doubly-linked list (\texttt{std::list}) of heartbeat times and \texttt{MPI\_Request} objects (for MPI message progression) are stored per replica, per tag value. I illustrate an example with two teams in Figure~\ref{fig:performance-consistency}, where team 0 is faster than team 1. Team 1 finally triggers the heartbeat operation $h_1$ with tag 2. This means the data can be sent back to team 0 where the receive had already been posted. Team 0 has advanced further through the execution and has already triggered both heartbeats for $h_2$ with a non-blocking send. However, the data will not be picked up by team 1 until it has also reached that point and triggered the receives.

\subsection{Ensuring data consistency with heartbeats}\label{sec:fault-tolerance}
\begin{algorithm}
	\caption{Compare consistency data between ranks for fault tolerance}\label{alg:fault-tolerance}
	\begin{algorithmic}[1]
		\Procedure{compareConsistency}{}
		\State \Call{compareProgress}{}(Algorithm~\ref{alg:progress})
		\State Hash the consistency data with \texttt{std::hash}
		\For {each other team}
		\State \texttt{Isend} hash data to rank in corresponding team
		\State Post \texttt{Irecv} for hash data from rank in corresponding team
		\EndFor
		\State \texttt{MPI\_Testsome} to check and progress received hashes
		\If{hashes are not equivalent}
		\State Start the recovery process
		\EndIf
		\EndProcedure
	\end{algorithmic}
\end{algorithm}

I now detail Algorithm~\ref{alg:fault-tolerance} which ensures data consistency between replicas. This is important for faults that do not cause a rank to stop (fail-stop) but instead cause it to make incorrect computations. Memory faults are one cause for this. The concept is similar to comparing the times among replicas. The only difference is that the user must supply a data buffer via the \texttt{*sendbuf} parameter of \texttt{MPI\_Sendrecv}. This could be the new solution of an iteration or any characteristic value. Data is then hashed (using \texttt{std::hash}) compared among replicas. I neglect the theoretical plausibility of hash collisions in this proof-of-concept. Tags can again be used to discern among different buffer checks alike comparing the times for multiple code sections among replicas. In fact the solution is almost identical. The values of $h$ in Figure~\ref{fig:performance-consistency} now also contain the hashes in addition to the heartbeat times.

If a fault is detected then what happens next depends on how many teams are used. For only two teams then there is no way to correct the error, as we do not know which team is at fault. The best solution here is to roll-back both teams if possible and recompute the data. If one team gets a different result from previously then it can be identified as faulty team. If three teams are used, a voting mechanism can tell which team needs to be replaced. It is not usually possible to identify a single rank of a team at fault as the calculation is for most codes contributed by other ranks. 

This approach is much more coarse-grained than existing approaches, which check the consistency of all MPI data in every function call. However, I claim that this is excessive, unnecessary and incurs too much overhead. As long as the solution or calculation is consistent per iteration then this implies that all the MPI data in between was also correct. The advantages of such an assumption far outweigh any potential edge-case scenarios. I now discuss how these benefit the overhead of the consistency scheme. 

\subsubsection{Overhead of the consistency scheme}

Importantly, the teams should be placed as far apart as possible within a cluster. This is the motivation behind the mapping of ranks to team ranks, which by default maps teams to contiguous portion of ranks. The ranks must also be continuously distributed on the native hardware, but this cannot be controlled by {\tmpi}. If the user wishes the teams to be even further apart, pinning of the ranks can be performed easily by most MPI libraries and batch schedulers. 

This logical topology provides two advantages: (i) increased resiliency against faults and (ii) eliminates the extra strain on the network hardware created by replication. The resiliency is increased as it is rare for a fault to spread from a single node, or a clustered set of nodes. Issues predominantly effect either a single node's hardware (e.g.\ DRAM failure) or hardware supplying a contained set of nodes (e.g.\ power or network switch failure)~\cite{baseman18dram,di18fatal}. 

One of the main issues of replication other than the increased hardware demands is that it is assumed that any replication will also have a negative impact on the performance. However, I claim that this not true under a few assumptions. 

\begin{figure}
	\centering
	\includegraphics[width=\textwidth]{figures/tmpi-rank-diagram.eps}
	\caption[{\tmpi} on a 2:1 fat tree network topology.]{An annotated overview of a \tmpi-enabled application with respect to a common 2:1 fat tree network topology. The circles represent ranks, in the form mapped / original rank. The squares represent switches at level \texttt{S$_{\texttt{level}}$}, where \texttt{S$_{\texttt{0}}$} represents the root switch.}\label{fig:tmpi-architecture}
\end{figure}

For most common network topologies, the intra-team (original application) messages do not overlap. This holds certainly for any tree-based topologies, with a 2:1 fat-tree example given in Figure~\ref{fig:tmpi-architecture}. The application is launched on 8 nodes/ranks, and {\tmpi} creates 2 teams of 4 ranks. Team 0 occupies nodes 0 to 3 and team 1 occupies nodes 4 to 7. Therefore, the bandwidth-heavy application-based network traffic is contained up to switches at level 1 (\texttt{S$_{\texttt{1}}$}). Only heartbeat messages cross the top-most switch \texttt{S$_{\texttt{0}}$} and overlap between the two teams. These are small, asynchronous, non-urgent messages issued once per application iteration (infrequently). 

The concept can easily be applied to other network topologies too. Provided that the underlying MPI library is also of good quality, the extra processes should also have no impact as all application communication is done via a per-team communicator. Heartbeat messages sent in a dedicated communicator are tiny and therefore non-critical. 

In summary, the overhead of the effective consistency scheme here is equal to the overhead of the heartbeat messages, essentially negligible. Variations on the fat tree topology are used everywhere in HPC clusters, from local machines like Hamilton at Durham University to Summit, the world's largest supercomputer to date~\cite{exaop2018}. They have provably efficient communication for general purpose use~\cite{leiserson1985fat}.


\subsection{Summary of capabilities}
\begin{table}
	\centering
	\caption[Feature comparison including {\tmpi}]{Feature comparison of existing rank replication approaches including {\tmpi}.\label{table:comparison-tmpi}}
	\begin{tabular}{l*4c}
		\toprule
		                            & RedMPI & echoMPI & SDR-MPI    & {\tmpi} \\
		\cmidrule(lr){1-5}
		Fixed replication           & \cmark & \cmark  & \cmark     & \cmark  \\
		Partial replication         & \cmark & \cmark  & &         \\
		Platform independent (PMPI) & \cmark & \cmark  & & \cmark  \\
		Error correction            & \cmark & \cmark  & & \cmark  \\
		Performance analysis        &        &         &  & \cmark  \\
		Work-sharing                &        &         & \cmark &         \\
		Overhead (1--5)              & 3/4    & 5       & 2          & 1       \\
		\bottomrule 
	\end{tabular}
\end{table}
With an understanding of the underlying library architecture, I summarise the capabilities based upon the number of teams and heartbeats per iteration:
\begin{enumerate}
	\item \textbf{Two} teams with a \textbf{single} heartbeat can identify a slow \textbf{team} and provide error \textbf{detection}.
	\item \textbf{Two} teams with \textbf{dual} heartbeats can identify a slow \textbf{rank} and provide error \textbf{detection}.
	\item \textbf{Three or more} teams with a \textbf{single} heartbeat can identify a slow \textbf{team} and provide error \textbf{correction} via check-pointing.
	\item \textbf{Three or more} teams with \textbf{dual} heartbeats can identify a slow \textbf{rank} and provide error \textbf{correction} via check-pointing.
\end{enumerate}
In reality the most effective configuration is the second, as the overhead of a dual heartbeat is negligible in comparison to the benefits. Although using three or more ranks does support error correction, the multiplication of resource usage might not justify its gain. It is highly likely that if a error is simply detected, then the application will just be started on a different set of nodes, with the offending nodes replaced. Check-pointing is an expensive operation in both time and resources. I summarise the other capabilities in comparison to the previous approaches from Section~\ref{section:lit-review} in Table~\ref{table:comparison-tmpi}. {\tmpi} omits partial replication as it has been shown to offer limited use for resiliency by James et al~\cite{elliott2012combining}. Instead, I offer a library that provides the highest performance, while retaining advanced resiliency and consistency features; all with minimal modification to existing application code. 

% \begin{}

\section{Results}\label{sec:tmpi:results}
In this section I showcase the capabilities of the {\tmpi} library with experiments based upon three increasingly complex applications:
\begin{enumerate}
	\item A classical ``ping-pong'' based acceptance test to investigate the basic bandwidth and latency overhead of {\tmpi}.
	\item A mini application (miniapp) designed to mimic the behaviour of conventional scientific computing applications.
	\item A complex {\exahype} application to show how {\tmpi} may be used in a real-world setting.  
\end{enumerate}
In all three cases, the only changes required were to link against {\tmpi} (no changes at compile time) and to insert one or two heartbeats with the \texttt{MPI\_Sendrecv} command as described in Section~\ref{sec:progress}. The number of teams is dictated by the \texttt{TMPI\_TEAMS} environment variable, read when when the application calls \texttt{MPI\_Init}. The applications are then launched using the chosen MPI library's command. If the common \texttt{mpiexec} command is used then the application is started using \texttt{mpiexec -np x*t} where \texttt{x} is the ranks per team and \texttt{t} is the number of teams. For example, if an application wishes to use three teams of ten ranks then the command would be \texttt{mpiexec -np 30}.


The experiments were carried out on the Hamilton 7 cluster at Durham University. Each node consists of 2 x Intel Xeon E5-2659 v4 (Broadwell) 12 core, 2.2 GHz processors. They also have 64 GB of TruDDR4 memory and are connected via an Intel Omnipath 100Gb interconnect in a 2:1 non-blocking fat tree topology.


\subsection{Ping Pong Test}
\begin{algorithm}
	\caption{Ping Pong acceptance test}\label{alg:ping-pong}
	\begin{algorithmic}[1]
		\Procedure{PingPongTest}{}
		\For {$t \rightarrow t_{\max}$}
		\State Call \texttt{MPI\_Sendrecv} heartbeat
		\For {$n_{\min} \rightarrow n_{\max}$}
		\State Start timer
		\For {$i \rightarrow i_{\max}$}
		\If {rank == 0}
		\State Send message of size $n$
		\State Receive message of size $n$
		\ElsIf {rank == 1}
		\State Receive message of size $n$
		\State Send message of size $n$
		\EndIf
		\EndFor
		\State Stop timer
		\State new bandwidth $\gets 2\cdot i_{\max} / $timer
		\If {new bandwidth $>$ bandwidth[$n$]}
		\State bandwidth[$n$] $\gets$ new bandwidth
		\EndIf
		\EndFor
		\EndFor
		\EndProcedure
	\end{algorithmic}
\end{algorithm}
The first experiment to carry out is a simple test to study how much performance is lost by replicating ranks. Previous examples from the literature suggest that it can have a large effect depending on the technique used. With a complete lack of synchronisation among ranks in {\tmpi}, it is reasonable to expect that the overhead will be negligible. The benchmark chosen is the same as the one used by~\cite{Ferreira2011rmpi,engelmann2011redundant} which measures the bandwidth and latency between ranks in a classic ``ping pong'' experiment~\cite{gropp1999reproducible}. The benchmark exchanges increasingly large messages between two ranks starting with only a message envelope as the payload (Algorithm~\ref{alg:ping-pong}). As the message size increases, the runtime is dictated by the bandwidth rather than the latency. If {\tmpi} has any effect on the message passing performance of a rank then it will be shown by an increase in the runtime. Although it is clear that reduced bandwidth will be noticed, a decrease in the latency will also be shown as $10^4$ messages are sent back and forth in each trial. 25 trials are performed per message size. The maximum bandwidth over all trials is taken. In this experiment only 2 ranks are required per team, where each team is placed on a separate node of the cluster. This simulates the topology in Figure~\ref{fig:tmpi-architecture} where intra-team communication does not overlap. The \texttt{tmi} fabric is used to ensure ranks do not communicate via the shared memory fabric. 

 
\begin{figure}%
	\centering
	\centering
	\subfloat[Bandwidth per team\label{fig:bandwidth-per-rank}]{{\includegraphics[width=.4\linewidth]{experiments/latency/bandwidth-per-rank} }}%
	\qquad
	\subfloat[Difference compared to baseline\label{fig:bandwidth-diff}]{{\includegraphics[width=.4\linewidth]{experiments/latency/bandwidth-diff} }}%
	\caption[Ping-pong benchmark results.]{A typical ``ping-pong'' stress test of the implementation where the bandwidth between two ranks is measured with increasing message size.}\label{fig:overhead}
\end{figure}%
The results in Figure~\ref{fig:bandwidth-per-rank} confirm no performance drop when splitting the original communicator and introducing more teams. Furthermore, the results in Figure~\ref{fig:bandwidth-diff} reinforce the statement that the performance of individual nodes can vary by a large amount. Take for example the experiment with two teams. The first team records a 5\% \emph{higher} bandwidth than the baseline of pure MPI for $10^4 < m < 10^5$, where $m$ is the message size in bytes. The second team however records 5\% \emph{lower} bandwidth for the same message sizes.
The main takeaway from this experiment is that it is valid to claim that {\tmpi} is a near zero-overhead solution to MPI rank replication, something the previous implementations are not able to. This is through the vast reduction in synchronisation between replicas. I now move onto assessing the capabilities of the heartbeat functionality. 

\subsection{A Typical Scientific Computing Miniapp}\label{sec:miniapp-results}
\begin{algorithm}
	\caption{Miniapp}\label{alg:miniapp}
	\begin{algorithmic}[1]
		\Procedure{miniapp}{}
		\For {$t = t_{\min} \rightarrow t_{\max}$}
		\State \texttt{MPI\_Barrier(MPI\_COMM\_WORLD)}
		\State First heartbeat: \texttt{MPI\_Sendrecv(..., 1, ..., MPI\_COMM\_SELF)}
		\For {$i = i_{\min} \rightarrow i_{\max}$}
		\State $\sin(1.0/3.0)$
		\EndFor
		\State Second heartbeat: \texttt{MPI\_Sendrecv(..., -1, ..., MPI\_COMM\_SELF)}
		\State \texttt{MPI\_Barrier(MPI\_COMM\_WORLD)}
		\EndFor
		\EndProcedure
	\end{algorithmic}
\end{algorithm}
The next experiment demonstrates the capabilities of the {\tmpi} library with regards to detecting slow teams or ranks. To do so a simple mini application (miniapp) was designed that only performs arbitrary flops in ``synchronised'' iterations. The simple algorithm is given in Algorithm~\ref{alg:miniapp}. If only one heartbeat is used then the second \texttt{MPI\_Sendrecv} is omitted (although it is irrelevant which is removed). This application is useful as it can operate with arbitrary numbers of ranks. It is an excellent proof-of-concept before moving onto real applications in Section~\ref{section:teams:exahype}. Since it can be safely assumed that the overhead introduced by {\tmpi} is near-zero, this experiment does not actually perform any communication but instead tests the viability of using heartbeats to detect slow ranks or teams. However, many applications do model this behaviour of iterations with communication followed by computation. 


A rank could be slow for a whole range of reasons, such as system load, network load or because it is about to fail. To simulate this the library includes functionality for a benchmark studying the properties of slow ranks, as such behaviour usually occurs non deterministically making it tricky to investigate organically. A signal handler for SIGUSR1 is registered within the library, such that when raised the rank will sleep for one second. The more often this signal is sent to a rank, the slower the progress through the work assigned to it. Therefore it effectively simulates a rank that is slow through more organic means. More sophisticated techniques exist such as lowering the frequency of a CPU~\cite{Treibig:10:Likwid}. These often require administrator privileges and the sleep command simulates effectively the same behaviour: a slow down of progress. Ultimately, for this test it is not important how the difference in heartbeat times is created.

\begin{figure}%
	\centering
	\subfloat[One heartbeat per iteration\label{fig:slow-rank-perf:single}]{{\includegraphics[width=.4\linewidth]{experiments/slow-replicas/perf-single-heartbeat/plots/constant-single} }}%
	\qquad
	\subfloat[Two heartbeats per iteration\label{fig:slow-rank-perf:double}]{{\includegraphics[width=.4\linewidth]{experiments/slow-replicas/perf-double-heartbeat/plots/constant-single} }}%
	\caption[Capabilities of one versus two heartbeats.]{An experiment with the benchmark defined in Algorithm~\ref{alg:miniapp}. A single rank is chosen to be ``slowed down'' with one second sleep commands sent every five seconds. The left is the difference in heartbeat times for a single heartbeat per iteration, where only slow teams can be detected. The right is the difference in heartbeat times for the two heartbeats per iteration. The slow down of rank 0 in team 1 can then be detected individually.}\label{fig:slow-ranks}
\end{figure}%

The first thing I investigated was the use of one versus two heartbeats per iteration (Figure~\ref{fig:slow-ranks}). For this test the same rank is sent the one second sleep signal every five seconds. This simulates where one rank is much slower than the rest, and the aim is to detect this slow rank. The benchmark based on Algorithm~\ref{alg:miniapp} was used with 100 iterations, and the time taken to execute $5\times10^7$ $\sin$ operations per iteration was $\approx 0.4$ seconds. Figure~\ref{fig:slow-rank-perf:single} shows the time between heartbeats for when only a single heartbeat per iteration is inserted. Even though only rank 0 in team 0 was sent the sleep signals, the library can only detect that both rank 0 \emph{and} rank 1 in team 0 were slower than their replicas in team 1. This is because rank 1 must wait for rank 0 at the \texttt{MPI\_Barrier} at the end of the iteration. This barrier simulates any kind of synchronisation such as neighbour communication. Therefore, it only hits the heartbeat once rank 0 has caught up. Importantly, {\tmpi} is able to detect the fault within this team. It took 1 second longer than the other team to compute the same amount of work. In Figure~\ref{fig:slow-rank-perf:double}, two heartbeats are inserted: one at the start of the work and another at the end as outlined in Algorithm~\ref{alg:miniapp}. This means that there are ranks synchronising between heartbeats. This is clearly visible in the results where this time rank 0 in team 1 was sent the signal every 5 seconds. With two heartbeats {\tmpi} is able to single out the slow rank which takes 1 second longer than its replica in team 0 to compute the same work. This is a powerful feature, and the future direction of this approach is outlined in Chapter~\ref{chapter:conclusions}.

\begin{figure}%
	\centering
	\captionsetup[subfigure]{justification=centering}
	\subfloat[\label{fig:perf-sim-grid:constant-single}][Selection: constant\newline Frequency: constant]{{\includegraphics[width=.3\linewidth]{experiments/slow-replicas/perf-double-heartbeat/plots/constant-single} }}%
	\quad
	\subfloat[\label{fig:perf-sim-grid:constant-rr}][Selection: round-robin\newline Frequency: constant]{{\includegraphics[width=.3\linewidth]{experiments/slow-replicas/perf-double-heartbeat/plots/constant-rr} }}%
	\quad
	\subfloat[\label{fig:perf-sim-grid:constant-random}][Selection: random\newline Frequency: constant]{{\includegraphics[width=.3\linewidth]{experiments/slow-replicas/perf-double-heartbeat/plots/constant-random} }}%
	\quad
	\subfloat[\label{fig:perf-sim-grid:increasing-single}][Selection: constant\newline Frequency: decreasing]{{\includegraphics[width=.3\linewidth]{experiments/slow-replicas/perf-double-heartbeat/plots/increasing-single} }}%
	\quad
	\subfloat[\label{fig:perf-sim-grid:increasing-rr}][Selection: round-robin\newline Frequency: decreasing]{{\includegraphics[width=.3\linewidth]{experiments/slow-replicas/perf-double-heartbeat/plots/increasing-rr} }}%
	\quad
	\subfloat[\label{fig:perf-sim-grid:increasing-random}][Selection: random\newline Frequency: decreasing]{{\includegraphics[width=.3\linewidth]{experiments/slow-replicas/perf-double-heartbeat/plots/increasing-random} }}%
	\quad
	\subfloat[\label{fig:perf-sim-grid:random-single}][Selection: constant\newline Frequency: random]{{\includegraphics[width=.3\linewidth]{experiments/slow-replicas/perf-double-heartbeat/plots/random-single} }}%
	\quad
	\subfloat[\label{fig:perf-sim-grid:random-rr}][Selection: round-robin\newline Frequency: random]{{\includegraphics[width=.3\linewidth]{experiments/slow-replicas/perf-double-heartbeat/plots/random-rr} }}%
	\quad
	\subfloat[\label{fig:perf-sim-grid:random-random}][Selection: random\newline Frequency: random]{{\includegraphics[width=.3\linewidth]{experiments/slow-replicas/perf-double-heartbeat/plots/random-random} }}%
	\caption[Simulating slow behaviour patterns on a representative miniapp.]{A series of nine experiments using Algorithm~\ref{alg:miniapp}. Ranks are sent a command to sleep for 1 second with a three different selection criteria and three different frequency intervals. The ``selection'' and ``frequency'' parameters are described in Section~\ref{sec:miniapp-results}.}\label{fig:perf-sim-grid}
\end{figure}%
The second experiment using the miniapp is designed to simulate a wide variety of potential misbehaviour by modifying two variables: to which rank the signal is sent and the frequency of the signals. 
\begin{enumerate}
	\item \textit{Constant}: select the same rank every time 
	\item \textit{Round robin}: select each rank in turn
	\item \textit{Random}: select rank at random
\end{enumerate}
and the time between signals is one of:
\begin{enumerate}
	\item \textit{Constant}: always wait a fixed time between signals
	\item \textit{Decreasing}: start with a maximum interval between signals then reduce by a fixed factor each time
	\item \textit{Random}: wait for a random time between signals
\end{enumerate}

These test cases were chosen as some of the combinations can be envisaged as real world scenarios. Others were included as no one really knows what the runtime behaviour of future hardware will be. However, the {\tmpi} library is well equipped to monitor any variations between ranks. For example constant selection with a constant interval simulates a slow rank as it will always lag behind the corresponding ranks in other teams. Constant selection and a decreasing interval simulates a failing rank and eventually will be declared dead. Constant selection with a random interval simulates a rank with sporadic performance, maybe being impeded by another application or event. Finally, random selection with a random interval can be seen as an exaggeration of a real HPC environment.

Figure~\ref{fig:perf-sim-grid} shows the results over the whole parameter space. In all cases {\tmpi} is able to detect the slow-down of individual ranks. I am confident that in real scenarios this statement holds. 


\subsection{A Real Application: LOH.1 simulation}\label{section:teams:exahype}
\begin{figure}%
	\centering
	\includegraphics[width=0.5\linewidth]{figures/loh_pic_cropped.png}
	\caption[LOH.1 visualisation. ]{Cut through the solution of the LOH.1 benchmark running on the {\exahype} engine. A point source induces an “earthquake” just below the surface. Waves propagate from this point but yield complicated patterns as the cubic domain contains two layers of different material~\cite{loh12006}.}\label{fig:loh1}
\end{figure}%

The next challenge for the implementation was how effective it would work with a ``real world'' application (Figure~\ref{fig:loh1}). The chosen set-up is a seismic benchmark simulation known as LOH.1 running on the {\exahype} engine~\cite{loh12006}. The runtime characteristics of the code are highly complex, featuring dynamic asynchronous communication and computation patterns. Adding heartbeats to the code was still trivial. The start beat is still added after the communication phase of the previous timestep and then the end beat is placed before any communication is waited upon. 

\begin{figure}%
	\centering
	\includegraphics[width=1.0\linewidth]{figures/trace-analyzer-heartbeat-annotated.eps}
	\caption[LOH.1 benchmark message profile.]{A profile of the benchmark code when running for three timesteps on 29 balanced ranks. Example heartbeat locations are marked by the magenta dashed line.}\label{fig:loh1-trace}
\end{figure}% 
Chapter~\ref{chapter:tasks} thoroughly details the {\exahype} work-flow but for our replication studies only a knowledge of the phases in Figure~\ref{fig:loh1-trace} is required. It begins with start-up phase where the grid is constructed. Then, at the beginning of each timestep the tasks for the timestep are spawned. Here the first heartbeat is placed. A barrier occurs at the end of the timestep where the code waits for the tasks spawned to complete. At the end of this barrier the second heartbeat is triggered. At no point between these heartbeat points does a rank wait for another as the communication barriers occur after the second heartbeat. A final clean-up phase mainly involves deallocating memory. For a simpler presentation of Figure~\ref{fig:loh1-trace} the heartbeats are shown aligned but was not the case for the real execution. I reiterate no synchronisation occurs between heartbeats. The communication does not cause any delays in this phase.


\begin{figure}%
	\centering
	\captionsetup[subfigure]{justification=centering}
	\subfloat[\label{fig:exa-grid:constant-single}][Selection: constant\newline Frequency: constant]{{\includegraphics[width=.3\linewidth]{experiments/slow-replicas/exahype/plots/constant-single} }}%
	\quad
	\subfloat[\label{fig:exa-grid:constant-rr}][Selection: round-robin\newline Frequency: constant]{{\includegraphics[width=.3\linewidth]{experiments/slow-replicas/exahype/plots/constant-rr} }}%
	\quad
	\subfloat[\label{fig:exa-grid:constant-random}][Selection: random\newline Frequency: constant]{{\includegraphics[width=.3\linewidth]{experiments/slow-replicas/exahype/plots/constant-random} }}%
	\quad
	\subfloat[\label{fig:exa-grid:increasing-single}][Selection: constant\newline Frequency: decreasing]{{\includegraphics[width=.3\linewidth]{experiments/slow-replicas/exahype/plots/increasing-single} }}%
	\quad
	\subfloat[\label{fig:exa-grid:increasing-rr}][Selection: round-robin\newline Frequency: decreasing]{{\includegraphics[width=.3\linewidth]{experiments/slow-replicas/exahype/plots/increasing-rr} }}%
	\quad
	\subfloat[\label{fig:exa-grid:increasing-random}][Selection: random\newline Frequency: decreasing]{{\includegraphics[width=.3\linewidth]{experiments/slow-replicas/exahype/plots/increasing-random} }}%
	\quad
	\subfloat[\label{fig:exa-grid:random-single}][Selection: constant\newline Frequency: random]{{\includegraphics[width=.3\linewidth]{experiments/slow-replicas/exahype/plots/random-single} }}%
	\quad
	\subfloat[\label{fig:exa-grid:random-rr}][Selection: round-robin\newline Frequency: random]{{\includegraphics[width=.3\linewidth]{experiments/slow-replicas/exahype/plots/random-rr} }}%
	\quad
	\subfloat[\label{fig:exa-grid:random-random}][Selection: random\newline Frequency: random]{{\includegraphics[width=.3\linewidth]{experiments/slow-replicas/exahype/plots/random-random} }}%
	\caption[Simulating slow behaviour patterns on the LOH.1 benchmark.]{The nine experiments from Figure~\ref{fig:perf-sim-grid} repeated with a seismic benchmark application running on the {\exahype} engine. The ``selection'' and ``frequency'' parameters are described in Section~\ref{sec:miniapp-results}. The markers on the scatter plots represent the team rank. The difference in heartbeat times for the first and second replica are plotted. If the first replica is detected to be slow then it is coloured red. If the second replica is detected to be slow then it is coloured green.}\label{fig:exa-grid}
\end{figure}%

The same experimental setup was modified from the previous section to work with the engine. This time 12 ranks per team were used, and the selection criteria definitions slightly modified. In the initial testing of the experiment I sent the sleep commands to different ranks to simulate a rank slowing down. However, in the engine there is a significant load imbalance in this setup as this is something yet to be tackled (see Chapter~\ref{section:teams:outlook} for some remarks on this). If any other ranks than rank 1 (in any team) are selected to be ``slowed-down'' via the sleep command then {\tmpi} will not notice. As rank 1 has the most work to do and the other ranks wait for its results at every timestep after the second heartbeat. Therefore, unless the rank is unrealistically slowed down (or killed) then the sleep command will be called after the work is completed and the end-beat executed. This highlights one potential issue with relying on heartbeats for detecting performance reductions. If such a fault occurs outside of the heartbeats {\tmpi} cannot detect a slowdown. However, the heartbeat paradigm is designed such that users can maximise the coverage to minimise this risk. With the proposal to balance tasks among teams more effectively in Chapter~\ref{chapter:conclusions}, the imbalances can be reduced leading to a much improved runtime. To ensure the slowdowns are noticeable by {\tmpi}, I modify the selection definitions of the benchmark from Section~\ref{sec:miniapp-results} to be as follows:
\begin{enumerate}
	\item \textit{Constant}: select rank 1 in the first team every time
	\item \textit{Round robin}: select rank 1 but in from a different team in a round-robin fashion each time. 
	\item \textit{Random}: select rank 1 each time but the team is random. 
\end{enumerate}

Additionally, I found that the sleep command interfered with some of the clean-up operations of the code, such as freeing memory. Therefore I only sent the sleep commands within a 45 second window. Clearly, these changes would not be necessary if I had access to more realistic testing methods.

{\tmpi} is still capable of detecting the various slow-downs of rank 1 (Figure~\ref{fig:exa-grid}). What is also noticeable is the increase in variance of the data. The heartbeat times in between vary much more so than the simple benchmark in the previous section. I attribute this to the profile of the code, which has complex characteristics in comparison to the well defined benchmark. 

This second experiment showcases the power of {\tmpi}. With two additional lines of code even in a complex code base such as {\exahype}, faults in either data or performance can easily be detected and reported by the library. I am confident that this approach can be easily integrated into most scientific codes and possibly even more general applications. Moreover, the addition of the heartbeat messages had no noticeable impact on the performance, validating this lightweight approach to ensuring consistency.

\section{Outlook}\label{section:teams:outlook}
In this chapter I have presented an MPI rank replication scheme. It improves over the numerous existing implementations. My {\tmpi} library is available as a C++ library that intercepts MPI calls through the dedicated profiling interface. By loosening temporal consistency constraints, replicas are able to operate completely asynchronously from each other. This reduces the performance overhead of replication to practically zero. I validate this claim through the classical ``ping-pong'' micro-benchmark which showed that increasing the number of replicas has no impact on the bandwidth or latency requirements. At application-specified intervals, called a heartbeat, the replicas exchange data and performance consistency information in a fully non-blocking fashion. This allows the {\tmpi} library to detect ranks that are slow, failing or producing erroneous results. I presented these capabilities first on a mini-application that simulates the runtime behaviour of many real applications in scientific computing. I show that the integration of {\tmpi} into a complex code base such as {\exahype} is trivial, and {\tmpi} continues to have excellent performance monitoring capabilities of applications with extremely dynamic runtime behaviour properties.

The {\tmpi} library has several areas for further research. These were not investigated here owing to the scope of the thesis. First, for real fault tolerance the {\tmpi} library should automatically swap out slow, failing or error producing ranks. Swapping is a complex process that is not supported by many MPI implementations. They exit at the first sign of a failing rank. However, techniques from research into run-through stabilisation techniques show such capabilities are feasible with custom MPI library support~\cite{bland2013ulfm}. Second, to showcase the capabilities better, real world failure scenarios should be simulated rather than the primitive ``sleep'' approach in Section~\ref{sec:miniapp-results}/\ref{section:teams:exahype}. This could be based on existing data provided by many HPC institutions~\cite{Schroeder2007,Schroeder2010}. A final area for future research is the automatic insertion of the heartbeats into the application code. For example, the heartbeats could be inserted between any two synchronising MPI calls. However, with the reduced temporal consistency of {\tmpi}, an implementation would have to make sure that the heartbeats were called by the ``same'' functions in all replicas. 

In summary, the {\tmpi} provides a valuable contribution to the existing area of rank replication. If a na\"ive state machine approach is neglected in favour of the fully asynchronous heartbeat based consistency method proposed in this chapter, advanced fault tolerance techniques can be leveraged transparently to application code with practically zero performance overhead.

In the final chapter of this thesis I bring together the two ideas proposed on tasks and teams. Although powerful concepts in their own right I show they can be combined to equalize work imbalances among individual ranks within a team.

